Answer Fast: Accelerating BERT on the Tensor Streaming Processor

Transformers have become a predominant machine learning workload, they are not only the de-facto standard for natural language processing tasks, but they are also being deployed in other domains such as vision and speech recognition. Many of the transformer-based applications are real-time systems such as machine translation and web search. These real time systems often come with strict end-to-end inference latency requirements. Unfortunately, while the majority of the transformer computation comes from matrix multiplications, transformers also include several non-linear components that tend to become the bottleneck during an inference. In this work, we accelerate the inference of BERT models on the tensor streaming processor. By carefully fusing all the nonlinear components with the matrix multiplication components, we are able to efficiently utilize the on-chip matrix multiplication units resulting in a deterministic tail latency of 130 $\mu$s for a batch-1 inference through BERT-base, which is 6X faster than the current state-of-the-art.

==> groqAPI.tex <==
\section{GroqAPI}
% DO NOT START THIS SECTION UNTIL THE REST OF THE PAPER IS FINISHED.
% I am not sure if we have space to add this section - probably not.
Most likely we will not have space for this section.
\begin{itemize}
\item While we have a full-fledged compiler (that takes in pytorch, tensorflow, etc..), there is always a need to give users more control over how they map their workload (reference NVIDIA equivelent, Cereberas SDK, etc..)
\item What does GAPI do? Raises the programming abstraction level of the TSP so that users don't get bogged down with details - automated decisions when possible, but give users the freedom for full control
\item scheduling
\item resource allocation
\item show a simple snippet of back-to-back buffered components and pipelined buffered components
\end{itemize}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
